Synthetic measurements of runaway electron synchrotron emission in the SPARC tokamak

With plasma currents up to 8.7 MA, the SPARC tokamak runs the risk of forming multi-MA beams of relativistic "runaway" electrons (REs) which could damage plasma facing components if unmitigated. The infrared (IR) and visible imaging and visible spectroscopy systems in SPARC are designed with measurements of synchrotron emission from REs in mind. Synchrotron radiation is emitted by REs along their direction of motion, opposite the plasma current. Matched clockwise and counterclockwise wide views are proposed to detect synchrotron and background radiation, allowing observation of RE synchrotron emission in both plasma current configurations. Due to SPARC's high toroidal magnetic field strength, 12.2 T on axis, the synchrotron light spectrum is expected to peak in the visible-IR wavelength range. The synthetic diagnostic tool SOFT (Synchrotron Orbit-Following Toolkit) is used to model synchrotron images and spectra for three scenarios, with appropriate magnetic equilibria for each: REs generated during plasma current ramp-up, steady-state flattop (although unlikely, but serving as a reference), and disruptions. Required time resolutions, achievable spatial coverage, and appropriate spectral ranges for various RE energies are assessed.

==> contributions.tex <==
\section*{Author contributions}\label{sec:contributions}

    RAT blah.

==> outline.tex <==
\section{Outline}
\begin{enumerate}
    \item Intro, REs, fig equilibrium (start-up, flattop, disruption)
    \item SPARC imaging/spectroscopy system, fig CW/CCW views, table of parameters: viewing direction, opening angle, spectral range, time resolution, pixels
    \item Flattop, scan in radius, pitch (0, 0.1, 0.2)
    \item Startup, scan in energy (0.1,1,10), spectral shift
    \item Disruption, scan in vertical position ()
    \item Summary, 
\end{enumerate}
